Self-supervised Learning on Graphs: Deep Insights and New Direction

The success of deep learning notoriously requires larger amounts of costly annotated data. This has led to the development of self-supervised learning (SSL) that aims to alleviate this limitation by creating domain specific pretext tasks on unlabeled data. Simultaneously, there are increasing interests in generalizing deep learning to the graph domain in the form of graph neural networks (GNNs). GNNs can naturally utilize unlabeled nodes through the simple neighborhood aggregation that is unable to thoroughly make use of unlabeled nodes. Thus, we seek to harness SSL for GNNs to fully exploit the unlabeled data. Different from data instances in the image and text domains, nodes in graphs present unique structure information and they are inherently linked indicating not independent and identically distributed (or i.i.d.). Such complexity is a double-edged sword for SSL on graphs. On the one hand, it determines that it is challenging to adopt solutions from the image and text domains to graphs and dedicated efforts are desired. On the other hand, it provides rich information that enables us to build SSL from a variety of perspectives. Thus, in this paper, we first deepen our understandings on when, why, and which strategies of SSL work with GNNs by empirically studying numerous basic SSL pretext tasks on graphs. Inspired by deep insights from the empirical studies, we propose a new direction SelfTask to build advanced pretext tasks that are able to achieve state-of-the-art performance on various real-world datasets. The specific experimental settings to reproduce our results can be found in \url{https://github.com/ChandlerBang/SelfTask-GNN}.

==> section/acknowledgements.tex <==
\begin{ack}
\toreword{Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare 
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.
Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.}
\end{ack}

==> section/broader_impact.tex <==
\section*{Broader Impact}
\toreword{Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
biases in the data. If authors believe this is not applicable to them, authors can simply state this.
Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}}

==> table/fewer_sample.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \caption{\comment{make this into a figure?}}
% \begin{tabular}{@{}cccc@{}}
% \multicolumn{4}{c}{\textbf{5 Sampler Per Class}}                                                                                  \\
%                 & \multicolumn{1}{c}{\textbf{Cora}} & \multicolumn{1}{c}{\textbf{Citeseer}} & \multicolumn{1}{c}{\textbf{Pubmed}} \\
% \textbf{GCN}    & 0.6925                            & 0.5883                                & 0.6669                              \\
% \textbf{M3S}    & 0.7304                            &                                       &                                     \\
% \textbf{LP+SMP} & \textbf{0.7494}                   & \textbf{0.6247}                       & \textbf{0.6771}                     \\
% \multicolumn{4}{c}{\textbf{10 Samples Per Class}}                                                                                 \\
%                 & \multicolumn{1}{c}{\textbf{Cora}} & \multicolumn{1}{c}{\textbf{Citeseer}} & \multicolumn{1}{c}{\textbf{Pubmed}} \\
% \textbf{GCN}    & 0.7660                            & 0.6321                                & 0.7275                              \\
% \textbf{M3S}    & 0.7710                            &                                       &                                     \\
% \textbf{LP+SMP} & \textbf{0.7940}                   & \textbf{0.6610}                       & \textbf{0.7309}                    
% \end{tabular}
% \end{table}



% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{@{}lllllll@{}}
% \textbf{}       & \multicolumn{3}{c}{\textbf{5 Samples Per Class   For Training}}                                                 & \multicolumn{3}{c}{\textbf{10 Samples Per Class   For Training}}                                                \\
%                 & \multicolumn{1}{c}{\textbf{Cora}} & \multicolumn{1}{c}{\textbf{Citeseer}} & \multicolumn{1}{c}{\textbf{Pubmed}} & \multicolumn{1}{c}{\textbf{Cora}} & \multicolumn{1}{c}{\textbf{Citeseer}} & \multicolumn{1}{c}{\textbf{Pubmed}} \\
% \textbf{GCN}    & 0.6925                            & 0.5883                                & 0.6669                              & 0.7660                            & 0.6321                                & 0.7275                              \\
% \textbf{M3S}    & 0.7304                            &                                       &                                     & 0.7710                            &                                       &                                     \\
% \textbf{LP+SMP} & \textbf{0.7494}                   & \textbf{0.6247}                       & \textbf{0.6771}                     & \textbf{0.7940}                   & \textbf{0.6610}                       & \textbf{0.7309}                    
% \end{tabular}
% \end{table}
